Efficient Valuation of SCR via a Neural Network Approach

As part of the new regulatory framework of Solvency II, introduced by the European Union, insurance companies are required to monitor their solvency by computing a key risk metric called the Solvency Capital Requirement (SCR). The official description of the SCR is not rigorous and has lead researchers to develop their own mathematical frameworks for calculation of the SCR. These frameworks are complex and are difficult to implement. Recently, Bauer et al. suggested a nested Monte Carlo (MC) simulation framework to calculate the SCR. But the proposed MC framework is computationally expensive even for a simple insurance product. In this paper, we propose incorporating a neural network approach into the nested simulation framework to significantly reduce the computational complexity in the calculation. We study the performance of our neural network approach in estimating the SCR for a large portfolio of an important class of insurance products called Variable Annuities (VAs). Our experiments show that the proposed neural network approach is both efficient and accurate.

==> accuracy.tex <==
\subsection{Accuracy}\label{sec:accuracy}
The accuracy results of Table \ref{tb:rel_err1} may misleadingly 
suggest that the Kriging method with the Spherical variogram model is 
always capable of providing very accurate interpolations. In the 
experiments of this section, we provide results on the accuracy of 
different methods that contradicts this hypothesis. 

For our experiments in this section, we replicated the experiments 
of Section \ref{sec:performance}  with sets of representative contracts 
that are produced from the set of representative contracts in Section \ref{sec:performance} 
by removing $100$, $200$, $400$, $600$ and $800$ \ac{VA} contracts 
at random. Table \ref{tb:rel_err4} presents the mean and the standard deviation 
of the relative error, in estimation of the delta value of the 
\ac{VA} portfolio, for each method in these experiments. 
The results of Table \ref{tb:rel_err4} show high variance values for the  
accuracy of the Kriging methods, 
which contradicts our hypothesis. Another interesting observation 
is that the IDW methods and the RBF 
methods with a Gaussian kernel, in comparison to the Kriging methods, 
have a lower variance value for the relative error. 


\begin{table}[!bt]
 \centering
 \begin{tabular}{|l|l|l|}
  \hline
  Method & Mean (\%) & STD (\%)\\ 
  \hline
  Kriging (Spherical) & $0.47$ & $1.76$\\ 
  \hline
  Kriging (Exponential) & $-0.58$ & $2.19$\\
  \hline 
  Kriging (Guassian) & $1109.02$ & $3289.81$\\
  \hline
  IDW (p = 1) & $9.14$ & $1.75$\\
  \hline 
  IDW (p = 10) & $13.14$ & $0.42$\\
  \hline
  IDW (p = 100) & $12.06$ & $0.23$\\ 
  \hline 
  RBF (Gaussian, $\epsilon = 1$) & $-1.78$ & $0.48$\\
  \hline
  RBF (Gaussian, $\epsilon = 10$) & $38.87$ & $1.42$\\
  \hline
  RBF(Multi-Quad, $\epsilon = 1$) & $-58.65$ & $16.84$\\
  \hline
  RBF(Multi-Quad, $\epsilon = 10$) & $-9.15$ & $3.56$\\
  \hline
 \end{tabular}
 \caption{Mean and standard deviation of relative error in estimation of delta value via each method.}
 \label{tb:rel_err4}
\end{table}


==> performance.tex <==
\subsection{Performance}\label{sec:performance}
In this set of experiments, our objective is to provide a 
fair comparison of accuracy and computational efficiency 
of each proposed estimation method when the k-prototype distance 
function of \citep{Gan13-2} is used. Since we allow the guaranteed value of 
\acp{VA} in the synthetic portfolio to be different than their 
account value, we have modified the distance function to the following. 

\begin{equation}\label{eq:k_dist}
 D(\mathbf{x}, \mathbf{y}, \gamma) = \sqrt{\sum_{h \in N}(\frac{{x_h - y_h}}{\max_h - \min_h})^2
 + \gamma \sum_{h \in C}\delta(x_{h}, y_{h})}
\end{equation}
where $N = \{\text{AV, GD, GW, maturity, age, withdrawal rate}\}$ is the set of numerical values and 
$C = \{ \text{gender, rider} \}$ is the set of categorical values.

Similar to \citep{Gan15, Gan13-2}, we choose $\gamma = 1$. Moreover, 
we form the set of representative contracts, via the sampling method of 
Section \ref{sec:sampling_method}, from all combinations of end points 
presented in Table \ref{tb:rep_contracts1}. Because 
of the constraints on the guaranteed values, some of the entries are 
duplicate, which we remove to obtain a sample of size $1800$.


\begin{table}[!bt]
 \centering
 \begin{tabular}{|l|l|}
  \hline
  & Experiment 1\\
  \hline
  Guarantee Type & \{GMDB, GMDB + GMWB\}\\ 
  \hline
  Gender & \{Male, Female\}\\
  \hline
  Age & $\{20, 30, 40, 50, 60\}$\\
  \hline 
  Account Value & $\{1e4, 1.25e5, 2.5e5, 3.75e5, 5e5\}$\\
  \hline
  Guarantee Value & $\{0.5e4, 3e5, 6e5\}$\\
  \hline 
  Withdrawal Rate & $\{0.04, 0.08\}$\\ 
  \hline 
  Maturity & $\{10, 15, 20, 25\}$\\
  \hline
 \end{tabular}
 \caption{Attribute values from which representative contracts are generated for experiments.}
 \label{tb:rep_contracts1}
\end{table}


In order to be thorough in our experiments and comprehensive in our analysis, we present the 
results for all variants of Kriging, \ac{IDW}, and \ac{RBF} methods. For Kriging, we choose to experiment 
with all three major variogram models, i.e., spherical, exponential, and gaussian. For \ac{IDW}, we choose 
to experiment with different choices of the power parameter to see the effect of this free parameter on the 
accuracy of results. For \ac{RBF}, we study two of the most popular radial functions, Gaussian and 
multi-quadratic, and for each type of radial function, we experimented with two choices for the free 
parameter $\epsilon$. In Table \ref{tb:rel_err1}, the relative error in estimation of 
the delta value of the portfolio is presented. The relative error for method $m$ is calculated as follows.

\begin{equation}
 \text{Err}_m = \frac{\Delta_m - \Delta_{MC}}{|\Delta_{MC}|}
\end{equation}
where $\Delta_{MC}$ is the estimated delta value of the portfolio computed by \ac{MC} simulations and $\Delta_m$ is the 
estimate delta value of the portfolio computed by method $m$. While two of the Kriging methods provide accurate estimates, 
the accuracy of \ac{IDW}, and multi-quadratic \ac{RBF} methods is moderate. One interesting observation is that 
the choice of variogram model has substantial impact on the accuracy of the method and it confirms the result of 
\citep{Gan13-2} that the spherical method provides the best accuracy. Another interesting observation is the effect of 
the free parameters $p$ and $\epsilon$ on the accuracy of the \ac{IDW} and \ac{RBF} methods. The results suggest that 
the effective use of either method requires a careful tuning of these free parameters. 



\begin{table}[!bt]
 \centering
 \begin{tabular}{|l|l|}
  \hline
  Method & Relative Error (\%)\\
  \hline
  Kriging (Spherical) & $-0.03$\\ 
  \hline
  Kriging (Exponential) & $-1.61$\\
  \hline 
  Kriging (Guassian) & $< -500$\\
  \hline
  IDW (p = 1) & $9.11$\\
  \hline 
  IDW (p = 10) & $13.12$\\
  \hline
  IDW (p = 100) & $11.99$\\ 
  \hline 
  RBF (Gaussian, $\epsilon = 1$) & $-1.79$\\
  \hline
  RBF (Gaussian, $\epsilon = 10$) & $37.89$\\
  \hline
  RBF(Multi-Quad, $\epsilon = 1$) & $-71.62$\\
  \hline
  RBF(Multi-Quad, $\epsilon = 10$) & $-10.86$\\
  \hline
 \end{tabular}
 \caption{Relative error in estimation of delta value via each method.}
 \label{tb:rel_err1}
\end{table}


Table \ref{tb:sim_time1} presents the running time of each algorithm in two scenarios: 1) estimating the delta value of the portfolio 
only 2) estimating the delta value of each \ac{VA} policy in the portfolio and summing them to get the delta value of 
the portfolio. While the former does not provide a granular view of the portfolio, the latter gives a more 
refined estimation process and allows for deeper analysis and insights. Note that the times 
in Table \ref{tb:sim_time1} represent only the time that it took to estimate the values once we knew the delta values 
of the representative contracts. To get the total simulation time, add $187$ seconds to these times, 
which is the time that it took to estimate the delta value of representative contracts via \ac{MC} simulations.
The results show the superiority of the proposed framework over \ac{MC} simulation (speed up $> 15\times$) 
except when Kriging is used for per policy estimation of delta. 
Because the \ac{IDW} and \ac{RBF} methods by definition require the estimation of the delta of each policy and sum the estimations to 
get the delta value of the portfolio, we can see that simulation times for these methods are approximately equal in the two presented 
scenarios. Moreover, these methods are more efficient than the Kriging method, which confirms our analysis in Section \ref{sec:sif}.



\begin{table}[!bt]
 \centering
 \begin{tabular}{|l|l|l|}
  \hline
  Method & Portfolio & Per Policy\\
  \hline
  MC & $10617$ & $10617$\\
  \hline
  Kriging (Spherical) & $312$ & $> 320000$\\ 
  \hline
  Kriging (Exponential) & $333$ & $> 320000$ \\
  \hline 
  Kriging (Guassian) & $383$ & $> 320000$\\
  \hline
  IDW (P = 1) & $285$ & $286$\\
  \hline 
  IDW (P = 10) & $288$ & $287$\\
  \hline
  IDW (P = 100) & $287$ & $301$\\ 
  \hline 
  RBF (Gaussian, $\epsilon = 1$) & $295$ & $306$\\
  \hline
  RBF (Gaussian, $\epsilon = 10$) & $294$ & $315$\\
  \hline
  RBF(Multi-Quad, $\epsilon = 1$) & $289$ & $289$\\
  \hline
  RBF(Multi-Quad, $\epsilon = 10$) & $297$ & $292$\\
  \hline
 \end{tabular}
 \caption{simulation time of each method to estimate the delta value. All times are in seconds.}
 \label{tb:sim_time1}
\end{table}

